Ubiquitous Robot Control Through Multimodal Motion Capture Using Smartwatch and Smartphone Data

We present an open-source library for seamless robot control through motion capture using smartphones and smartwatches. Our library features three modes: Watch Only Mode, enabling control with a single smartwatch; Upper Arm Mode, offering heightened accuracy by incorporating the smartphone attached to the upper arm; and Pocket Mode, determining body orientation via the smartphone placed in any pocket. These modes are applied in two real-robot tasks, showcasing placement accuracy within 2 cm compared to a gold-standard motion capture system. WearMoCap stands as a suitable alternative to conventional motion capture systems, particularly in environments where ubiquity is essential. The library is available at: www.github.com/wearable-motion-capture.

==> glossary.tex <==
\newacronym{gyro}{\ensuremath{\bm{\phi}}}{gyroscope measurements}
\newacronym{grav}{\ensuremath{\bm{\gamma}}}{gravity sensor}
\newacronym{lacc}{\ensuremath{\bm{\alpha}}}{linear acceleration sensor}
\newacronym{racc}{\ensuremath{\bm{\alpha}_\mathrm{raw}}}{raw acceleration}
\newacronym{swrot}{\ensuremath{\bm{\theta}}}{virtual rotation vector sensor}
\newacronym{swrot_calib}{\ensuremath{\bm{\theta}_c}}{calibration forward-facing direction}
\newacronym{pres}{\ensuremath{\rho}}{atmospheric pressure sensor}
\newacronym{rot_hip}{\ensuremath{\textbf{q}_\mathrm{h}}}{hip rotation}
\newacronym{rot_larm}{\ensuremath{\textbf{q}_\mathrm{l}}}{lower arm rotation}
\newacronym{rot_uarm}{\ensuremath{\textbf{q}_\mathrm{u}}}{upper arm rotation}
\newacronym{rot_larm_r}{\ensuremath{\textbf{q}^r_\mathrm{l}}}{relative lower arm rotation}
\newacronym{rot_uarm_r}{\ensuremath{\textbf{q}^r_\mathrm{u}}}{relative upper arm rotation}
\newacronym{6drr}{6DRR}{six-dimensional rotation representation}
